Always on Voting: A Framework for Repetitive Voting on the Blockchain

Elections repeat commonly after a fixed time interval, ranging from months to years. This results in limitations on governance since elected candidates or policies are difficult to remove before the next elections, if needed, and allowed by the corresponding law. Participants may decide (through a public deliberation) to change their choices but have no opportunity to vote for these choices before the next elections. Another issue is the peak-end effect, where the judgment of voters is based on how they felt a short time before the elections. To address these issues, we propose Always on Voting (AoV) -- a repetitive voting framework that allows participants to vote and change elected candidates or policies without waiting for the next elections. Participants are permitted to privately change their vote at any point in time, while the effect of their change is manifested at the end of each epoch, whose duration is shorter than the time between two main elections. To thwart the problem of peak-end effect in epochs, the ends of epochs are randomized and made unpredictable, while preserved within soft bounds. These goals are achieved using the synergy between a Bitcoin puzzle oracle, verifiable delay function, and smart contracts.

==> sec/AnonymousIdentity.tex <==
\st{In our scheme, we employ wallet addresses to keep track of authorized participants.
The map between participant $P$ and her wallet, recorded by the $EA$ is to prevent sybil attack (preventing any unauthorized person from voting) and double voting. For this reason, $EA$ is trusted to keep this mapping private. Only voters corresponding to white-listed wallets by $EA$ are allowed to vote and everyone else is blocked from voting on the smart contract. The wallet address corresponds to a unique random string associated with the voter. Its knowledge provides no additional information to the $EA$, since the $EA$ knows voter identities.

The AoV framework permits participants to change their vote at any time. 
The effect of the change is manifested at the end of the epoch when the tally is computed.  
However, $Adv_{net}$ can observe the vote transactions on $SC$ even though the vote choice remains confidential (preserving the privacy of votes). 
A participant might vote in one interval and then vote again in a future interval. 
$Adv_{net}$ cannot distinguish whether the participant voted again for the same candidate or changed her vote to a different
candidate due to assumed confidentiality-preserving properties of plugged voting protocols }%end st
(see \autoref{sec:underlying-voting-protocol}) %\ih{I'd not go into details of SOME specific plugged protocols that are using blinding keys. We should abstract from it, and also save the space.}.
%\sarad{agreed. commented out.}}
\st{However, both votes may be mapped to the same participant's blockchain wallet address if utilized naively, hence $Adv_{net}$ can determine how many times a participant voted.


To break the map between participant $P$ and her blockchain wallet address, we use the idea presented in type 2 deterministic wallets\footnote{See \url{https://en.bitcoin.it/wiki/BIP_0032}.}.
The objective is to synchronize a practically unlimited number of wallet public keys PKs (one per vote) between $EA$ and $P$ such that this PK list can be regenerated only by these two parties, while the corresponding private keys SKs can be computed only by $P$.
As mentioned in }%end st
\autoref{ssec:advmodel}, \st{$EA$ is assumed to verify identities honestly, and it supplies their corresponding wallet addresses to $SC$. 
The wallet address is generated as a function $f$ of the elliptic curve public key. 
Once the public key is available, it is straightforward to compute the corresponding wallet address.
Let $BP$ be the base point on the elliptic curve.
Further, let $PK$ be the blockchain wallet public key corresponding to a private key $SK$.
Here, $SK$ is chosen as a random positive integer whose size is bounded to the order of $BP$ on the chosen elliptic curve modulo a prime number. 
Note that } %end st
\autoref{eqn_anon01} -- \autoref{eqn_anon05}  
\st{ are computed off-chain.
As an illustration, let the first PK be computed as}%end st
\begin{equation}\label{eqn_anon01}
 \stkout{PK_{0} = SK_{0}\cdot BP},
\end{equation}
\st{and the next PK be}
\begin{equation}\label{eqn_anon02}
\stkout{PK_{1} = PK_{0}+SK_{1}\cdot BP.}
\end{equation}
%Also, 
%$A1_{SK} = A0_{SK}+A1_{SK}$.
\st{From} \autoref{eqn_anon01} \st{and}~\autoref{eqn_anon02}\st{, we observe that}
\begin{equation}\label{eqn_anon03}
 \stkout{(SK_{0}+SK_{1})\cdot BP = PK_{1}}.
\end{equation}
%
\st{The following steps ensue:}
\begin{compactenum}[i)]
	\item \st{During the identity verification, $P$ sends to $EA$:
	\textit{a}) wallet public key $PK_{0}$, \textit{b}) a random shared secret key $hk$, and \textit{c}) parameters $(g,p)$, where $g$ is a randomly chosen generator in $F_p^{*}$ (i.e., a prime field)  and $p$ is a large prime.
   The wallet address is a public function of the wallet public key.
%   \sarad{it sounds like PK is the name of the wallet. a bit confusing, changed to public key.} 
   Hence, $EA$ computes $W_{0}=f(PK_0)$ and stores it.}
	
	\item \st{The private key of $P$ at any future voting epoch $e=\{1,2,3,...,2^{128}-1\}$  is generated by $P$ as   }
	\begin{equation}\label{eqn_anon04}
	SK_{e}= SK_{0} + HMAC_{hk}(g^e),
	\end{equation}
	\st{where $g^e\in F_p^{*}$ is the output of pseudo-random number generator (PRNG) in epoch $e$, HMAC$(.)$ is HMAC-X-256 using shared secret key ${hk}$ between $EA$ and $P$, which is unknown to $Adv_{net}$ and serves for stopping her from mapping $P$'s wallet addresses.}
	
	\item \st{The corresponding $PK$ of $P$ for epoch $e$ is }  
	
	\begin{equation}\label{eqn_anon05}
	PK_{e}= PK_{0} + HMAC_{hk} (g^e)\cdot BP.
	\end{equation}
\end{compactenum} 
%
\st{$EA$ and $P$ can compute $PK_e$ but $SK_e$ is held only by $P$.
This effectively separates PKs from their SKs and, at the same time, maps it to $P$'s first wallet public key, i.e., $PK_{0}$.   
At any voting iteration $e$, the public key $PK_{e}$, and the corresponding wallet address can be computed by both $EA$ and $P$.
Since the shared secret $hk$ used with HMAC is known only to $EA$ and $P$, no third party, including $Adv_{net}$, is able to compute any future PKs. 
Hence, for a sequence of wallet addresses of $P$  given by $W_{e}$ = $f(PK_{e})$, the map between the wallet address and $P$ is broken for all other parties other than $EA$ and $P$.} 

\subsubsection*{\textbf{\st{Batching the Requests}}}
\st{It is important to note that if a participant wishes to change her vote within the same voting interval, she should submit the request with the new wallet address to $EA$ who will approve the request in batches (aggregating multiple such requests) in order to improve the resistance against mapping of former wallet addresses to new ones.
In detail, the $EA$ will mark all former addresses as \textit{invalid} and approve the new ones within a single transaction.}
%the $EA$ is required to set participant $P’$s previous wallet address to “invalid” to prevent double voting  (in the same interval) whenever $P$ submits her new wallet address to continue voting. 
%
%This allows $Adv_{net}$ to  possibly link the two wallets.
%The link made by $ADV_{net}$ are strongest when only one participant changed her vote in the same voting interval.
%A participant who values maximum wallet privacy must change her vote only during the next (or a future) interval. In any future interval, all participants use a new wallet address to send their vote transactions to the blockchain. Since all participant wallet addresses have changed, $ADV_{net}$ is no longer able to link wallets.
%\ih{this sentence is still unclear --``employing a revote'' does not give any clue to reader.}
%\sarad{updated sentences above.}
%
\st{In the extreme case, when a batch contains only one participant (who wanted to change her vote), $Adv_{net}$ can map the two wallets.
Therefore, such a participant should value her wallet privacy and vote only once during the next interval (or alternatively change her address again and be a part a bigger batch).
%
%In case a participant votes more than once in an interval, her wallet addresses (used in that interval) may be linked by $Adv_{net}$, but only the $EA$ knows the true identity of the wallet address holder (i.e., participant). 
Using VPN/dVPNs may further limit the $Adv_{net}$'s ability to map participant IP addresses.}

==> sec/boothsharding.tex <==

\subsection{Privacy Implications of Booth Sharding}
\label{ssec:shardinganalysis}

\begin{figure*}
	\centering
	%	\subfloat[Booth size=30, $p=0.6$]{
	%		\includegraphics[width=0.5\textwidth]{fig/pdfpngp0.pdf}
	%	}
	%	\subfloat[Booth size=100, $p=0.6$]{
	%		\includegraphics[width=0.5\textwidth]{fig/pdfpngp1.pdf}
	%	}
	%	\newline
	\subfloat[][Booth size X=30 participants, candidate winning \ensuremath{p=0.9}]{
		\includegraphics[width=0.5\textwidth]{fig/pdfpngp2.pdf}
	}
	\subfloat[][Booth size X=100 participants, candidate winning \ensuremath{p=0.9}]{
		\includegraphics[width=0.5\textwidth]{fig/pdfpngp3.pdf}
	}
	
	
	\caption{Binomial probability distribution function of X booth participants voting for their favorite candidate whose winning probability is $p$. 
		%		\IH{The figure does not make sense to me -- how P that 25 participants choose the same candidate can be lower than in the case of 35?}
		%		\sarad{Fig updated for 100 particpants, its due to the nature of binomial pdf. }
	}
	\label{fig:binomialpdf}
	
\end{figure*}

The global tally is computed by the aggregator smart contract as the sum of individual booth contract tallies (see Fig.~\ref{fig:booth} and Fig.~\ref{fig:model}).
A common way to eliminate demographic voting bias is to randomly assign participants to a booth.
Even so, there is a small probability that all booth participants voted for the same candidate (hence revealing their vote).
This event is more significant when the winning probability of one candidate is much higher than the others.
Fig.~\ref{fig:binomialpdf} gives the probability that X  participants in a booth, voted for the same candidate, given the candidate winning probability.


Fig.~\ref{fig:binomialpdf}(a) represents a booth with 30 participants and candidate winning probability, $p=0.9$. The probability that all participants assigned to a booth, voted for the same candidate is 
$P(30,X=30,p=0.9)\stackrel{\sim}{=} 0.0423$.
Fig.~\ref{fig:binomialpdf}(b) represents a booth with 100 participants and candidate winning probability, $p=0.9$. The probability that all participants in a booth voted for the same candidate is 
$P(100,X=100,p=0.9)\stackrel{\sim}{=} 0.00003$.
While the probabilities in the booth with 100 participants are lower, this may not be sufficient.
\ih{I am not sure whether this subsection has any value in the current form. The point is that you are currently interested only in the event of voting for the same choice. However, even if all participants do not vote for the same vote there is an information saying that every participant from the booth voted for the winning choice with the probability equal to e.g., 0.9, which needs to be considered as well. So, maybe we should not deal with this issue at all and rely on the annonimization technique that preclude linking of the real identity with the vote/blockchain address.}

For example, consider  an election with 1 million participants.
Let $boothsize =30$ and $numbooths = \lceil(1000000/30)\rceil =33334$.
We know $P(30,X=30,p=0.9)\stackrel{\sim}{=} 0.0423$.
The number of booths where all participants likely voted for the same candidate is $0.0423\cdot33334 \simeq 1410$ (in 33334 booths).
This may be unacceptably high. The booth size is increased from 30 to 100 participants. Then, $P(100,X=100,p=0.9)\stackrel{\sim}{=} 0.00003$.
The number of booths where all participants  likely voted for the same candidate is reduced to
$0.00003\cdot 10000=0.3$ (in 10000 booths).
In this manner, a suitable booth size may be determined at an acceptable probability limit.



==> sec/pseudocode.tex <==

\begin{algorithm}[t]
	\label{alg:vdfdeposit}
	\DontPrintSemicolon
	
	\footnotesize
	\SetKwProg{Fn}{Function}{:}{\KwRet}
	\SetKwFunction{VDFADD}{VdfAdd}
	
	% Write Function with word ``Def''
	\SetKwProg{Fn}{Def}{:}{}
	\Fn{\VDFADD{\st{$y, \pi, blockheight$}}}{	
		\st{writeState}(\st{$``vdfadd"~||~ blockheight, y~||~\pi$})	
	}
	\caption{\st{VDF Add}}
\end{algorithm}



\begin{algorithm}[t]
	\label{alg:bpodeposit}
	\DontPrintSemicolon
	\footnotesize
	
	\SetKwProg{Fn}{Function}{:}{\KwRet}
	\SetKwFunction{BPOAdd}{BpoAdd}
	
	% Write Function with word ``Def''
	\SetKwProg{Fn}{Def}{:}{}
	\Fn{\BPOAdd{\st{$Target, BH, blockheight$}}}{	
		\st{writeState($``bpoadd"~||~ blockheight,BH~||~Target$)\\	
		writeState($``blockheightStored",blockheight$)\\
		writeState($``blockheader"~||~blockheight,BH$)}
	}
	\caption{\st{BPO Add}}
\end{algorithm}



\st{
The high-level functionality of the AoV framework and its smart contracts is shown in} Algorithm~\autoref{alg:framework}\st{, and the trigger mechanism is presented in }Algorithm~\autoref{alg:trigger}.
Algorithm~\ref{alg:framework} \st{comprises of 5 main functions --- \textit{setup, registration, voting, tally} and \textit{revote}. 
The system parameters agreed upon are added by $EA$ using the \textit{setup} function of the smart contract. 
The $EA$ is also responsible for adding the list of valid participants' wallet addresses to the contract through the  \textit{registration} function.
The \textit{voting} function is supplied by a participant's wallet address, blinded vote, and its proof of correctness. 
This information is signed with $P_i$'s private key and sent to the contract. 
The \textit{voting} function carries out the necessary verifications and adds her vote. The participant wallet address is set to ``voted'' to disallow its reuse. 
Before invoking the \textit{tally} function, the VDF prover and BPO store their respective data to the contract (see} Algorithm~\ref{alg:vdfdeposit} and Algorithm~\ref{alg:bpodeposit}). 
\st{Next, the \textit{tally} function is called by $EA$ or any authorized participant. 
%The prover has access to all public Bitcoin network information, results of VDF computation, and its proof. 
The \textit{tally} function carries out two main tasks. First, it checks whether the condition to trigger the interval tally is satisfied (see} Algorithm~\ref{alg:trigger}). \st{The second task (when triggered) is to tally the votes and return the results.
%\footnote{Note that instead of computing the tally, the contract can just verify the submitted tally to be correct, which is much cheaper than the tally computation.}
%Sarad. This would depend on the voting algorithm plugged-in. it is a specific detail. moved to comments.
%The implementation details are left to the reader.
When a participant wishes to vote again, she sends her next wallet address (synchronized with $EA$) to the \textit{revote} function.
The $EA$ will verify the new wallet address offline and call the \textit{registration} function to set the new address to valid (preferably in batches as mentioned in} \autoref{ssec:Anonid}). 
\st{Next, a participant may call the function \textit{Voting} and vote using her new wallet address.}
%While different voting protocols may be used with this framework,  resolving the dependencies needed to complete the tally is left to the voting implementation. \ih{Unimportant here.}

\begin{algorithm}[t]
	\label{alg:trigger}
	
	\DontPrintSemicolon
	\footnotesize
	
	\SetKwProg{Fn}{Function}{:}{\KwRet}
	\SetKwFunction{FTrigger}{VerifyTrigger}
	
	% Write Function with word ``Def''
	\SetKwProg{Fn}{Def}{:}{}
	\Fn{\FTrigger{\st{$y, \pi, T, BH, params\_struct$}}}{	
%		$y$ = $vdf$\;
	\st{	$b$ = -$1$\\
		%\ih{Where is params\_struct from? Add to input?}\\
		$tt$ = readState($params\_struct.totaltime$)\\ 
		$ft$ = readState($params\_struct.ft$)\\
		$seed$ = readState($params\_struct.key$)\\  
		$IntervalTime$ = $tt/ft$\\ 
		$BHsInInterval$ = $IntervalTime/10$}\\
		
		\If{\st{$SHA256(BH)<T$} } 
		{
			\If{ \st{$Verify\_VDF(y,\pi)==True$}}
			{
				\st{$a = SHA(y)$}\;
				$b = a (mod\; BHsInInterval)$\\			
			}
		}
		\If{\st{b==0}}
		{
			\KwRet \st{$True$}\;
		}
		\Else{\KwRet \st{$False$}\;}
	}
	
	
	\caption{\st{Trigger Mechanism}}
\end{algorithm}

%Sarad: i commented out BBB below and moved the BBB citation elsewhere.
%n some voting algorithms (e.g., BBB-voting~\cite{venugopalan2021bbbvoting}), they use multiparty computation to enable its self-tallying properties.
%Here, the blinding key information of each participant is mixed across all the registered participants. All participants must vote for a tally to be computed. Otherwise, a recovery round is initiated to remove faulty participants who did not vote and then compute the tally.
%Nevertheless, this section presents a high-level description of the AoV framework.
\begin{algorithm*}
	\label{alg:framework}
	
	\footnotesize
	% Set Function Names
	\SetKwFunction{FMain}{Main}
	\SetKwFunction{FSetup}{Setup}
	\SetKwFunction{FReg}{Registration}
	\SetKwFunction{FVoting}{Voting}
	\SetKwFunction{FTally}{Tally}
	\SetKwFunction{FRevote}{Revote}
	
	\KwInput{\st{Set1: $\forall$ participants $P_i$, wallet addresses $(WA_{ij})$, blinded vote $BV_{ij}$ (by $P_i$ for her $j^{th}$ voting occurence,  $j=0,1,2,3,...$) \& zero knowledge proof of vote correctness ($ZKP_{ij}$), $booth_{no}$. Set2: system parameters $init\_params$, BTC blockheader $BH$, $VDF(BH)$, proof $\pi$, BTC target $T$, BTC blockheight.}}
	\KwOutput{\st{Total tally of votes in the interval.}}
	%\KwData{Testing set $x$}
	
	\medskip
	% Write Function with word ``Function''
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\FSetup{\st{$init\_params$}}}%\tcp{$init_{params}$: Agreed upon system parameters. }
	{
		\st{writeState($params\_struct, init\_params$)} \tcp{\st{add system parameters as key-value pairs into $params\_struct$.}}
		%b = second\;
		%sum = first + second\;
		%\KwRet $params\_{str}$\
	}
	\smallskip
%	\;
	
	% Write Function with word ``Function''
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\FReg{\st{$msg1=WA_{ij}, msg2=valid\_flag, EA\_signed\_msg$}}}{
		%Load system parameters ($init_{params}$) for voting.\\
		\st{$msg = msg1~||~msg2$} \tcp{\st{concatenate message parts.}}
		\st{$EA\_{pubkey}$=} \st{readState($params\_struct.EA\_public\_key$)} \tcp{\st{get $EA$ public key.}}
		
		\If{\st{VerifySig$(msg,EA\_signed\_msg, EA\_{pubkey})=True$}}
		{
			\If{\st{$valid\_{flag}==True$}}
			{
				\st{writeState($WA_{ij},``valid"$)} \tcp{\st{set wallet address to valid.}}
			}
			\Else
			{
				\st{writeState($WA_{ij},``invalid"$)} \tcp{\st{set wallet address to invalid.}}
				
			}
		}
		%sum = first + second\;
		%\KwRet $init\_params$\;
	}
	\smallskip
%	\;
	
	
	
	% Write Function with word ``Function''
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\FVoting{\st{$msg1=WA_{ij},msg2=BV_{ij},msg3=ZKP_{ij},P_i\_signed\_msg$}}}{
		\st{$msg = msg1~||~msg2~||~msg3$\\
		$wallet\_status$= readState($WA_{ij}$)\\
		$P_i\_{pubkey}$= readState($params\_struct.P_i\_public\_key$)\\
		$sig\_flag$ = VerifySig($msg$,$P_i\_signed\_msg$,$P_i\_{pubkey}$)\\
		$zkp\_flag$ = VerifyZKP($BV_{ij},ZKP_{ij}$)}\\
		
		\If{\st{($sig\_flag$ and $zkp\_flag$) == $True$ and $wallet\_status==``valid"$ }}
		{
			\st{writeState($``vote"~||~WA_{ij},BV_{ij}$)} \tcp{\st{The latest wallet address of $P_i$ is mapped to her private vote. The key  in (key,value) is prefixed with `vote' tag to identify valid votes w.r.t. wallet addresses.}}
			\st{writeState($WA_{ij},``voted"$)} \tcp{\st{set $WA$ to voted \& prevent voting from that address again.}}
			
			
		}
	}
	\smallskip
%	\;
	
	
	
	
	% Write Function with word ``Function''
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\FTally{\st{$blockheight$}}}{
		\st{$total\_tally=-1$\\
		$stored\_blockheight$ = readState($``blockheightStored"$)}\tcp{\st{\textit{blockheightStored} is from} Algorithm~\ref{alg:bpodeposit}: \st{BPO Add.}}
		\st{$BH=$readState($``blockheader"~||~blockheight$)}\tcp{\textit{\st{blockheight}} \st{is the argument passed to the function Tally.}}
		\st{$y,\pi$ = readState($``vdfadd"~||~blockheight$)}\tcp{\textit{\st{vdfadd}} \st{is read from Algorithm}~\ref{alg:vdfdeposit}.}
		\st{$BH,Target$ = readState($``bpoadd"~||~blockheight$)\\
		$trigger\_flag$=VerifyTrigger($y, \pi, Target,BH, params\_struct$)}\tcp{ \st{Call Algorithm}~\autoref{alg:trigger}.}
		\If{(\st{$stored\_blockheight$ == $blockheight$}) \st{and $trigger\_flag$ == True}}
		{
			
			\st{$total\_tally = \sum\limits_{no=1}^{X\cdot Y} local\_tally(booth_{no})$}\\
			%writeState($params\_struct.blockheight, blockheight$)	
			
		}
		\KwRet $total\_{tally}$		
	}
	\smallskip
%	\;
	
	% Write Function with word ``Function''
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\FRevote{\st{$msg=WA_{ij}, P_i\_signed\_msg$}}}{
		\st{$P_i\_{pubkey}$= readState($params\_struct.P_i\_public\_key$)} \tcp{\st{get $P_i$ public key}}
		
		\If{\st{VerifySig$(msg,P_i\_signed\_msg, P_i\_{pubkey})=True$}}
		{
			\st{writeState($WA_{ij},``pending"$)} \tcp{\st{set wallet address to pending verification by $EA$.}}
		}
		\tcp{\st{Next, $EA$  calls $Registration()$, where it sets a new wallet address of $P_i$ to valid.}}
		\tcp{\st{Further, $P_i$ calls $Voting()$ to re-vote using the new wallet address.}}
		
		%sum = first + second\;
		%\KwRet $init\_params$\;
	}
	
	
	\caption{\st{Always on Voting Framework}}
\end{algorithm*}





